Learning Novel Objects Continually Through Curiosity

Children learn continually by asking questions about the concepts they are most curious about. With robots becoming an integral part of our society, they must also learn unknown concepts continually by asking humans questions. The paper analyzes a recent state-of-the-art approach for continual learning. The paper further develops a self-supervised technique to find most of the uncertain objects in an environment by utilizing the cluster representation of the previously learned classes. We test our approach on a benchmark dataset for continual learning on robots. Our results show that our curiosity-driven continual learning approach beats random sampling and softmax-based uncertainty sampling in terms of classification accuracy and the total number of classes learned.

==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}

talk about continual learning approaches in general. but rather focus on the fact that this is not realistic. I would focus more on continual learning scenarios because this paper is more about the scenario... and then the algorithm to solve the problem is just adapt CBCL-PR...
